PART: Pre-trained Authorship Representation Transformer

Authors writing documents imprint identifying information within their texts: vocabulary, registry, punctuation, misspellings, or even emoji usage. Previous works use hand-crafted features or classification tasks to train their authorship models, leading to poor performance on out-of-domain authors. Using stylometric representations is more suitable, but this by itself is an open research challenge. In this paper, we propose PART, a contrastively trained model fit to learn \textbf{authorship embeddings} instead of semantics. We train our model on ~1.5M texts belonging to 1162 literature authors, 17287 blog posters and 135 corporate email accounts; a heterogeneous set with identifiable writing styles. We evaluate the model on current challenges, achieving competitive performance. We also evaluate our model on test splits of the datasets achieving zero-shot 72.39\% accuracy when bounded to 250 authors, a 54\% and 56\% higher than RoBERTa embeddings. We qualitatively assess the representations with different data visualizations on the available datasets, observing features such as gender, age, or occupation of the author.

==> tables/tab_1_zeroshot.tex <==
\begin{table*}[htb]
\small
\begin{center}
\caption{Table with accuracy and top-5 accuracy relating $N$ authors to their original texts for five methods. (Values in parenthesis is the respective standard deviation of 100 repeats.)}\label{tab:results}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lr|llllll@{}}
\toprule
 & \textbf{}      & N=10          & N=20           & N=40           & N=60           & N=80           & N=100           \\ \midrule
\multirow{2}{*}{\textbf{Our method}}    & Top-1 Accuracy & 88.8\% (10.75)  & 86.72\% (10.74) & 84.27\% (10.53) & 82.28\% (10.23) & 80.81\% (9.84)  & 79.47\% (9.6) \\
 & Top-5 Accuracy & 99.1\% (2.59) & 98.16\% (3.49) & 96.9\% (4.16)  & 95.74\% (4.51) & 94.81\% (4.62) & 93.99\% (4.74)  \\ \midrule
\multirow{2}{*}{\textbf{RoBERTa-large}~\cite{liu2019roberta}} & Top-1 Accuracy & 68.85\% (14.71) & 65.49\% (13.54) & 62.45\% (12.86) & 59.66\% (12.71) & 57.71\% (12.21) & 56\% (11.9)   \\
 & Top-5 Accuracy & 89.4\% (7.56) & 86.08\% (8.13) & 82.83\% (8.87) & 79.96\% (9.59) & 77.74\% (9.86) & 75.94\% (10.01) \\ \midrule
\multirow{2}{*}{\textbf{XLM-RoBERTa-large}~\cite{conneau2019xlmroberta}} & Top-1 Accuracy & 66.6\% (13.18) & 62.5\% (13.4)  & 58.64\% (13.4) & 55.7\% (13.16)  & 53.57\% (12.71) & 51.72\% (12.41) \\
& Top-5 Accuracy & 90.15\% (6.46) & 86.26\% (7.92) & 82.06\% (9.78) & 78.76\% (10.68) & 76.18\% (11.02) & 74.08\% (11.27) \\ \midrule
\multirow{2}{*}{\textbf{DeBERTa-v3-large}~\cite{he2021debertav3}} &Top-1 Accuracy & 63.65\% (13.01) & 60.16\% (12.25) & 56.79\% (11.97) & 54.37\% (11.64) & 52.12\% (11.54) & 50.44\% (11.33) \\
&Top-5 Accuracy & 87.05\% (6.71)  & 83.32\% (8.02)  & 79.49\% (9.11)  & 76.64\% (9.8)   & 74.25\% (10.2)  & 72.19\% (10.52) \\  \midrule
\multirow{2}{*}{\textbf{Megatron-BERT}~\cite{narayanan2021efficient}} & Top-1 Accuracy & 68.75\% (14.89) & 65.7\% (14.22) & 62.71\% (13.54) & 59.53\% (13.51) & 57.3\% (13.04) & 55.47\% (12.69) \\
&Top-5 Accuracy & 91.7\% (6.21)   & 88.79\% (7.19) & 85.8\% (8.27)   & 83.06\% (9.08)  & 80.68\% (9.65) & 78.67\% (9.99) \\
\bottomrule
\end{tabular}%
}
\end{center}

\end{table*}
